Bright Extragalactic ALMA Redshift Survey (BEARS) III: Detailed study of emission lines from 71 Herschel targets

We analyse the molecular and atomic emission lines of 71 bright Herschel-selected galaxies between redshifts 1.4 to 4.6 detected by the Atacama Large Millimetre/submillimetre Array. These lines include a total of 156 CO, [C I], and H2O emission lines. For 46 galaxies, we detect two transitions of CO lines, and for these galaxies we find gas properties similar to those of other dusty star-forming galaxy (DSFG) samples. A comparison to photo-dissociation models suggests that most of Herschel-selected galaxies have similar interstellar medium conditions as local infrared-luminous galaxies and high-redshift DSFGs, although with denser gas and more intense far-ultraviolet radiation fields than normal star-forming galaxies. The line luminosities agree with the luminosity scaling relations across five orders of magnitude, although the star-formation and gas surface density distributions (i.e., Schmidt-Kennicutt relation) suggest a different star-formation phase in our galaxies (and other DSFGs) compared to local and low-redshift gas-rich, normal star-forming systems. The gas-to-dust ratios of these galaxies are similar to Milky Way values, with no apparent redshift evolution. Four of 46 sources appear to have CO line ratios in excess of the expected maximum (thermalized) profile, suggesting a rare phase in the evolution of DSFGs. Finally, we create a deep stacked spectrum over a wide rest-frame frequency (220-890 GHz) that reveals faint transitions from HCN and CH, in line with previous stacking experiments.

==> ALMA SGP emission line paper (Copy)/Derivedproperties2.tex <==
\begin{table}
    \centering
    \caption{Derived properties of the BEARS sample}
    \label{tab:extensiveTableOfAllProperties}
    \scalebox{0.86}{
    \begin{tabular}{lccccccccc}\hline
         ID & $\mu L_\mathrm{IR}$ & $\mu M_\mathrm{dust}$ & $\mu L^\prime_\mathrm{CO(1-0)}$ & $\mu M_\mathrm{H_2(CI)}$ & $\mu M_\mathrm{H_2(CO)}$ & $M_\mathrm{dyn}$ & $\Sigma_\mathrm{M_{H_2}(CI)}$ & $\Sigma_\mathrm{M_{H_2}(CO)}$ & $\Sigma_\mathrm{SFR}$ \\
        & $[10^{12}~\mathrm{L}_\odot]$ & $[10^{10}~\mathrm{M}_\odot]$ & $[10^{10}~\mathrm{K~km~s^{-1}~pc^2}]$ & $[10^{11}~\mathrm{M}_\odot]$ & $[10^{11}~\mathrm{M}_\odot]$ & $[10^{11}~\mathrm{M}_\odot]$ & $[10^4~\mathrm{M_\odot~pc^{-2}}]$ & $[10^4~\mathrm{M_\odot~pc^{-2}}]$ & $[10^2~\mathrm{M_\odot~yr^{-1}~kpc^{-2}}]$ \\\hline
        11&$66.4 $&$13.6 $&$58.9\pm10.9 $&$- $&$23.6\pm4.4 $&$1.5\pm0.3 $&$- $&$15.9 \pm 3.0 $&$6.6 \pm 1.7$\\
14&$97.8 $&$20.1 $&$52.9\pm14.5 $&$11.8\pm1.7 $&$21.2\pm5.8 $&$1.4\pm0.3 $&$2.2\pm0.3 $&$3.9 \pm 1.1 $&$2.6 \pm 0.7$\\
18&$58.0 $&$11.9 $&$40.7\pm11.5 $&$9.7\pm1.1 $&$16.3\pm4.6 $&$0.9\pm0.3 $&$2.4\pm0.3 $&$3.1 \pm 0.6 $&$2.1 \pm 0.5$\\
21&$45.8 $&$9.4 $&$76.1\pm43.5 $&$- $&$30.4\pm17.4 $&$4.9\pm2.2 $&$- $&$3.1 \pm 0.9 $&$1.4 \pm 0.4$\\
22&$50.8 $&$10.4 $&$61.3\pm25.4 $&$- $&$24.5\pm10.2 $&$7.5\pm3.7 $&$- $&$5.3 \pm 2.2 $&$1.6 \pm 0.4$\\
24&$56.7 $&$11.6 $&$20.9\pm4.0 $&$11.4\pm1.6 $&$8.3\pm1.6 $&$1.1 \pm 0.3 $&$27.7\pm3.9 $&$20.3 \pm 3.8 $&$20.2 \pm 5.1$\\
25&$59.8 $&$12.3 $&$78.2\pm33.1 $&$- $&$31.3\pm13.2 $&$1.3\pm0.5 $&$- $&$1.1 \pm 0.2 $&$0.6 \pm 0.1$\\
27&$98.6 $&$20.2 $&$79.7\pm32.7 $&$- $&$31.9\pm13.1 $&$2.7\pm1.0 $&$- $&$13.1 \pm 5.4 $&$6.0 \pm 1.5$\\
28&$71.8 $&$14.7 $&$85.2\pm51.5 $&$- $&$34.1\pm20.6 $&$7.5\pm2.7 $&$- $&$2.1 \pm 0.7 $&$1.4 \pm 0.3$\\
36&$77.5 $&$15.9 $&$23.6\pm6.9 $&$- $&$9.4\pm2.7 $&$1.2\pm0.3 $&$- $&$25.1 \pm 7.3 $&$30.3 \pm 7.6$\\
37&$29.7 $&$6.1 $&$34.7\pm16.7 $&$- $&$13.9\pm6.7 $&$4.8\pm2.1 $&$- $&$0.8 \pm 0.2 $&$0.4 \pm 0.1$\\
39&$46.7 $&$9.6 $&$33.7\pm9.7 $&$- $&$13.5\pm3.9 $&$9.3\pm5.9 $&$- $&$0.9 \pm 0.3 $&$0.5 \pm 0.1$\\
40&$22.0 $&$4.5 $&$16.2\pm4.5 $&$- $&$6.5\pm1.8 $&$2.6\pm0.6 $&$- $&$14.3 \pm 4.0 $&$7.1 \pm 1.8$\\
41&$47.1 $&$9.7 $&$18.9\pm6.0 $&$4.6^* $&$7.5\pm2.4 $&$2.6\pm0.7 $&$3.5^* $&$5.7 \pm 1.8 $&$5.3 \pm 1.3$\\
42&$27.8 $&$5.7 $&$38.9\pm23.9 $&$- $&$15.6\pm9.5 $&$4.0\pm0.9 $&$- $&$4.4 \pm 1.6 $&$2.4 \pm 0.6$\\
45&$13.2 $&$2.7 $&$10.8\pm2.7 $&$8.1\pm1.4 $&$4.3\pm1.1 $&$0.2\pm0.1 $&$19.1\pm3.2 $&$10.1 \pm 2.5 $&$4.5 \pm 1.1$\\
47&$25.0 $&$5.1 $&$21.6\pm8.4 $&$4.3\pm0.8 $&$8.6\pm3.4 $&$6.9\pm3.6 $&$0.5\pm0.1 $&$1.0 \pm 0.4 $&$0.4 \pm 0.1$\\
49A&$21.6 $&$4.4 $&$37.1\pm19.0 $&$- $&$14.8\pm7.6 $&$1.0\pm0.2 $&$- $&$0.6 \pm 0.2 $&$0.2 \pm 0.1$\\
49B&$8.8 $&$1.8 $&$8.4\pm3.7 $&$- $&$3.4\pm1.5 $&$1.1\pm0.5 $&$- $&$8.3 \pm 3.7 $&$3.2 \pm 0.8$\\
55&$19.3 $&$4.0 $&$16.3\pm3.6 $&$- $&$6.5\pm1.4 $&$1.8\pm0.6 $&$- $&$0.8 \pm 0.2 $&$0.3 \pm 0.1$\\
56C&$6.6 $&$1.4 $&$10.2\pm2.4 $&$- $&$4.1\pm0.9 $&$0.5\pm0.2 $&$- $&$9.8 \pm 2.3 $&$2.3 \pm 0.6$\\
57&$46.8 $&$9.6 $&$36.6\pm10.4 $&$- $&$14.7\pm4.2 $&$1.3\pm0.4 $&$- $&$3.2 \pm 0.9 $&$1.5 \pm 0.4$\\
60&$39.0 $&$8.0 $&$27.4\pm7.9 $&$- $&$11.0\pm3.2 $&$3.1\pm1.6 $&$- $&$1.4 \pm 0.4 $&$0.7 \pm 0.2$\\
63&$21.0 $&$4.3 $&$9.9\pm2.2 $&$5.4\pm0.8 $&$3.9\pm0.9 $&$1.7\pm0.5 $&$2.8\pm0.4 $&$2.0 \pm 0.5 $&$1.6 \pm 0.4$\\
68&$29.2 $&$6.0 $&$68.7\pm29.1 $&$- $&$27.5\pm11.6 $&$0.9\pm0.3 $&$- $&$36.4 \pm 7.7 $&$10.6 \pm 2.6$\\
69A&$15.2 $&$3.1 $&$19.5\pm4.0 $&$6.2\pm0.6 $&$7.8\pm1.6 $&$1.3\pm0.5 $&$4.2\pm0.4 $&$5.3 \pm 1.1 $&$1.5 \pm 0.4$\\
69B&$12.1 $&$2.5 $&$2.1\pm0.8 $&$1.4\pm0.4 $&$0.9\pm0.3 $&$0.08\pm0.01 $&$3.2\pm0.9 $&$1.9 \pm 0.7 $&$4.0 \pm 1.0$\\
73&$34.3 $&$7.0 $&$26.3\pm11.0 $&$- $&$10.5\pm4.4 $&$3.3\pm1.6 $&$- $&$8.7 \pm 3.6 $&$4.2 \pm 1.0$\\
77&$22.4 $&$4.6 $&$22.2\pm4.3 $&$3.6^* $&$8.9\pm1.7 $&$5.1\pm1.4 $&$1.2^* $&$3.0 \pm 0.6 $&$1.1 \pm 0.3$\\
80A&$6.3 $&$1.3 $&$14.5\pm3.5 $&$2.6^* $&$5.8\pm1.4 $&$2.1\pm0.2 $&$6.0^* $&$13.2 \pm 3.2 $&$2.1 \pm 0.5$\\
80B&$6.4 $&$1.3 $&$4.1\pm1.3 $&$- $&$1.6\pm0.5 $&$2.3\pm1.0 $&$- $&$0.2 \pm 0.1 $&$0.1 \pm 0.0$\\
81A&$11.4 $&$2.3 $&$27.7\pm8.6 $&$- $&$11.1\pm3.4 $&$2.1\pm1.4 $&$- $&$29.8 \pm 9.3 $&$4.5 \pm 1.1$\\
81B&$12.4 $&$2.5 $& $9.4\pm2.3 $&$- $&$3.7\pm0.9 $&$3.0\pm1.1 $&$- $&$9.0 \pm 2.2 $&$4.4 \pm 1.1$\\
86c&$29.5 $&$6.0 $&$28.7\pm5.6 $&$- $&$11.5\pm2.2 $&$3.2\pm1.0 $&$- $&$4.1 \pm 0.8 $&$1.5 \pm 0.4$\\
90&$41.3 $&$8.5 $&$26.1\pm8.1 $&$25.1\pm6.1 $&$10.4\pm3.2 $&$2.2\pm0.8 $&$3.8\pm0.9 $&$1.6 \pm 0.5 $&$0.9 \pm 0.2$\\
93&$27.6 $&$5.7 $&$18.8\pm4.6 $&$7.2\pm1.3 $&$7.5\pm1.8 $&$6.5\pm3.7 $&$1.6\pm0.3 $&$1.7 \pm 0.4 $&$0.9 \pm 0.2$\\
102&$21.1 $&$4.3 $&$21.4\pm6.7 $&$- $&$8.6\pm2.7 $&$1.1\pm0.6 $&$- $&$5.6 \pm 1.8 $&$2.0 \pm 0.5$\\
103&$23.6 $&$4.8 $&$30.9\pm12.7 $&$- $&$12.3\pm5.1 $&$1.6\pm0.8 $&$- $&$31.8 \pm 13.1 $&$8.9 \pm 2.2$\\
106&$29.7 $&$6.1 $&$18.8\pm4.0 $&$4.4\pm0.8 $&$7.5\pm1.6 $&$3.6\pm2.9 $&$1.2\pm0.2 $&$2.1 \pm 0.4 $&$1.2 \pm 0.3$\\
107&$18.9 $&$3.9 $&$16.8\pm3.6 $&$- $&$6.7\pm1.4 $&$0.8\pm0.3 $&$- $&$1.0 \pm 0.2 $&$0.4 \pm 0.1$\\
111&$22.7 $&$4.6 $&$29.6\pm6.0 $&$7.5\pm0.8 $&$11.9\pm2.4 $&$6.7\pm2.9 $&$1.2\pm0.1 $&$2.0 \pm 0.4 $&$0.6 \pm 0.1$\\
117&$39.8 $&$8.2 $&$25.9\pm11.0 $&$- $&$10.4\pm4.4 $&$2.5\pm0.8 $&$- $&$3.3 \pm 1.4 $&$1.9 \pm 0.5$\\
120A&$18.5 $&$3.8 $&$10.7\pm4.3 $&$- $&$4.3\pm1.7 $&$2.0\pm0.8 $&$- $&$11.4 \pm 4.6 $&$7.3 \pm 1.8$\\
120B&$18.2 $&$3.7 $&$6.7\pm3.1 $&$- $&$2.7\pm1.2 $&$8.9\pm5.1 $&$- $&$0.4 \pm 0.1 $&$0.6 \pm 0.1$\\
121&$27.0 $&$5.5 $&$32.8\pm10.1 $&$4.5^* $&$13.1\pm4.1 $&$3.3\pm1.0 $&$0.4^* $&$1.3 \pm 0.4 $&$0.4 \pm 0.1$\\
122A&$6.3 $&$1.3 $&$13.9\pm5.8 $&$- $&$5.5\pm2.3 $&$0.6\pm0.3 $&$- $&$14.1 \pm 5.9 $&$2.4 \pm 0.6$\\
123&$22.4 $&$4.6 $&$22.7\pm4.6 $&$10.3\pm1.3 $&$9.1\pm1.8 $&$3.5\pm1.3 $&$0.4\pm0.1 $&$0.4 \pm 0.1 $&$0.13 \pm 0.03$\\
131B&$15.7 $&$3.2 $&$5.9\pm1.8 $&$10.3\pm0.9 $&$2.4\pm0.7 $&$6.2\pm2.3 $&$4.8\pm0.4 $&$0.8 \pm 0.2 $&$1.1 \pm 0.3$\\
132&$16.7 $&$3.4 $&$19.3\pm4.1 $&$3.4\pm0.6 $&$7.7\pm1.7 $&$2.8\pm1.4 $&$1.1\pm0.2 $&$2.5 \pm 0.5 $&$0.8 \pm 0.2$\\
135A&$17.1 $&$3.5 $&$12.4\pm3.1 $&$2.9\pm0.5 $&$5.0\pm1.3 $&$1.8\pm0.6 $&$1.1\pm0.2 $&$1.8 \pm 0.5 $&$0.9 \pm 0.2$\\
138B&$23.6 $&$4.8 $&$3.7\pm0.7 $&$- $&$1.5\pm0.3 $&$0.07\pm0.02 $&$- $&$3.2 \pm 0.6 $&$7.5 \pm 1.9$\\
141&$16.0 $&$3.3 $&$20.8\pm5.1 $&$10.6\pm1.7 $&$8.3\pm2.0 $&$0.6\pm0.2 $&$23.6\pm3.7 $&$18.5 \pm 4.5 $&$5.2 \pm 1.3$\\
145&$13.8 $&$2.8 $&$19.9\pm4.5 $&$- $&$8.0\pm1.8 $&$8.2\pm2.0 $&$- $&$1.2 \pm 0.3 $&$0.3 \pm 0.1$\\
146B&$8.8 $&$1.8 $&$10.7\pm3.1 $&$- $&$4.3\pm1.3 $&$3.7\pm1.6 $&$- $&$0.5 \pm 0.1 $&$0.14 \pm 0.03$\\
155&$34.7 $&$7.1 $&$21.0\pm8.6 $&$- $&$8.4\pm3.5 $&$0.7\pm0.4 $&$- $&$0.9 \pm 0.4 $&$0.5 \pm 0.1$\\
159A&$14.0 $&$2.9 $&$19.1\pm3.7 $&$2.3\pm0.5 $&$7.6\pm1.5 $&$1.6\pm0.7 $&$0.10\pm0.02 $&$0.3 \pm 0.1 $&$0.08 \pm 0.02$\\
159B&$4.8 $&$1.0 $&$3.2\pm0.9 $&$1.7^* $&$1.3\pm0.3 $&$0.6\pm0.2 $&$3.8^* $&$2.9 \pm 0.8 $&$1.6 \pm 0.4$\\
160&$50.5 $&$10.4 $&$19.4\pm6.1 $&$7.2\pm1.8 $&$7.8\pm2.4 $&$2.9\pm0.7 $&$1.7\pm0.4 $&$1.8 \pm 0.6 $&$1.7 \pm 0.4$\\
163A&$6.5 $&$1.3 $&$4.3\pm1.6 $&$- $&$1.7\pm0.6 $&$0.7\pm0.3 $&$- $&$4.6 \pm 1.7 $&$2.6 \pm 0.6$\\
168&$49.2 $&$10.1 $&$17.1\pm3.6 $&$- $&$6.9\pm1.5 $&$11.1\pm3.0 $&$- $&$0.8 \pm 0.2 $&$0.9 \pm 0.2$\\
178A&$14.1 $&$2.9 $&$16.4\pm3.3 $&$- $&$6.5\pm1.3 $&$5.0\pm2.2 $&$- $&$1.1 \pm 0.2 $&$0.4 \pm 0.1$\\
178B&$9.9 $&$2.0 $&$14.2\pm3.0 $&$- $&$5.7\pm1.2 $&$8.2\pm2.7 $&$- $&$0.6 \pm 0.1 $&$0.16 \pm 0.04$\\
178C&$6.2 $&$1.3 $&$7.6\pm2.1 $&$- $&$3.0\pm0.8 $&$0.6\pm0.3 $&$- $&$7.4 \pm 2.1 $&$2.2 \pm 0.6$\\
182&$21.8 $&$4.5 $&$15.7\pm3.9 $&$7.2\pm1.2 $&$6.3\pm1.6 $&$3.8\pm1.1 $&$15.7\pm2.5 $&$13.7 \pm 3.4 $&$7.0 \pm 1.7$\\
184&$28.6 $&$5.9 $&$21.6\pm6.1 $&$6.0\pm0.9 $&$8.7\pm2.5 $&$0.5\pm0.2 $&$14.3\pm2.0 $&$20.6 \pm 5.8 $&$10.0 \pm 2.5$\\
189&$29.0 $&$6.0 $&$27.4\pm7.9 $&$- $&$10.9\pm3.2 $&$2.6\pm0.9 $&$- $&$0.8 \pm 0.2 $&$0.3 \pm 0.1$\\
200&$16.7 $&$3.4 $&$11.4\pm2.7 $&$4.8\pm1.3 $&$4.6\pm1.1 $&$0.8\pm0.4 $&$10.8\pm3.0 $&$10.2 \pm 2.5 $&$5.5 \pm 1.4$\\
207&$22.5 $&$4.6 $&$26.5\pm3.1 $&$- $&$10.6\pm1.2 $&$3.2\pm1.0 $&$- $&$2.7 \pm 0.3 $&$0.8 \pm 0.2$\\
208A&$15.7 $&$3.2 $&$17.0\pm4.5 $&$5.6\pm0.8 $&$6.8\pm1.8 $&$6.9\pm2.7 $&$2.4\pm0.4 $&$2.9 \pm 0.8 $&$1.0 \pm 0.2$\\
208B&$10.8 $&$2.2 $&$11.7\pm2.8 $&$3.4^* $&$4.7\pm1.1 $&$2.5\pm1.3 $&$8.0^* $&$11.0 \pm 2.7 $&$3.8 \pm 0.9$\\
209&$13.6 $&$2.8 $&$10.8\pm2.5 $&$- $&$4.3\pm1.0 $&$6.6\pm0.8 $&$- $&$0.3\pm 0.1 $&$0.14 \pm0.04$\\\hline
    \end{tabular}
    }
\raggedright \justify \vspace{-0.2cm}
\textbf{Notes:} $^*$ Calculated from $3\sigma$ upper limits shown in Table~\ref{tab:upperlimitsAdditional}
\end{table}

==> ALMA SGP emission line paper (Copy)/table_with_lines.tex <==
\begin{table}
    \caption{Spectral line luminosities from the stacked spectrum.}
    \label{tab:faintLines}
\centering
    \begin{tabular}{lccccclcccc}\hline 
    Line & Frequency & Sources & Line luminosity & S/N &  & Line & Frequency & Sources & Line luminosity & S/N  \\ 
     & [GHz] &  & [$10^9~\mathrm{K~km~s^{-1}~pc}^2$] & & & & [GHz] &  & [$10^9~\mathrm{K~km~s^{-1}~pc}^2$] \\ \hline
CO~(2--1) & 230.5380 & 2 & $\boldsymbol{ 129.3 \pm 14.9}$ & (9.9$\sigma$)  & & H$_2$O$^+$~607 & 607.2273 & 20 & $-0.1$ $\pm$ 1.1 & ($-0.1\sigma$) \\
CO~(3--2) & 345.7960 & 42 & $\boldsymbol{ 98.1 \pm 6.1}$ & (37.9$\sigma$)  & & H$_2$O$^+$~631 & 631.7241 & 17 & $-0.6$ $\pm$ 1.0 & ($-0.5\sigma$) \\
CO~(4--3) & 461.0408 & 35 & $\boldsymbol{ 74.2 \pm 4.4}$ & (53.8$\sigma$)  & & H$_2$O$^+$~634 & 634.2729 & 17 & $-0.8$ $\pm$ 1.1 & ($-0.7\sigma$) \\
CO~(5--4) & 576.2679 & 27 & $\boldsymbol{ 69.4 \pm 4.0}$ & (68.0$\sigma$)  & & H$_2$O$^+$~721 & 721.9274 & 6 & $-2.5$ $\pm$ 1.5 & ($-1.7\sigma$) \\
CO~(6--5) & 691.4731 & 10 & $\boldsymbol{ 50.5 \pm 3.1}$ & (40.1$\sigma$)  & & H$_2$O$^+$~742 & 742.1090 & 5 & 1.4 $\pm$ 1.5 & (1.0$\sigma$) \\
CO~(7--6) & 806.8984 & 4 & $\boldsymbol{ 38.2 \pm 2.6}$ & (25.6$\sigma$)  & & H$_2$O$^+$~746 & 746.5417 & 5 & $\boldsymbol{ 5.0 \pm 1.4}$ & (3.8$\sigma$) \\
$^{13}$CO~(2--1) & 220.3987 & 1 & 7.3 $\pm$ 18.4 & (0.4$\sigma$)  & & H$_2$O$^+$~761 & 761.8188 & 6 & 0.2 $\pm$ 1.2 & (0.2$\sigma$) \\
$^{13}$CO~(3--2) & 330.5880 & 41 & 4.3 $\pm$ 3.2 & (1.4$\sigma$)  & & LiH~(1--0) & 443.9529 & 30 & $-2.4$ $\pm$ 1.7 & ($-1.5\sigma$) \\
$^{13}$CO~(4--3) & 440.7652 & 28 & 2.2 $\pm$ 2.0 & (1.1$\sigma$)  & & CH~532 & 532.7239 & 34 & $\boldsymbol{ 6.8 \pm 1.2}$ & (5.8$\sigma$) \\
$^{13}$CO~(5--4) & 550.9263 & 29 & 1.6 $\pm$ 1.2 & (1.4$\sigma$)  & & CH~536 & 536.7614 & 31 & $\boldsymbol{ 7.8 \pm 1.3}$ & (6.5$\sigma$) \\
$^{13}$CO~(6--5) & 661.0673 & 14 & 1.2 $\pm$ 1.2 & (1.0$\sigma$)  & & OH~425 & 425.0363 & 25 & 0.4 $\pm$ 2.5 & (0.2$\sigma$) \\
$^{13}$CO~(7--6) & 771.1841 & 7 & $-0.9$ $\pm$ 1.0 & ($-0.9\sigma$)  & & OH~446 & 446.2910 & 31 & 2.5 $\pm$ 1.5 & (1.6$\sigma$) \\
$^{13}$CO~(8--7) & 881.2728 & 2 & $-1.2$ $\pm$ 1.5 & ($-0.8\sigma$)  & & CN~(N = 3--2) & 340.2478 & 41 & 2.1 $\pm$ 2.8 & (0.8$\sigma$) \\
C$^{18}$O~(2--1) & 219.5603 & 1 & $-24.3$ $\pm$ 19.8 & ($-1.2\sigma$)  & & CN~(N = 4--3) & 453.6067 & 36 & 2.2 $\pm$ 1.4 & (1.6$\sigma$) \\
C$^{18}$O~(3--2) & 329.3305 & 42 & 2.7 $\pm$ 3.2 & (0.9$\sigma$)  & & CN~(N = 5--4) & 566.9470 & 26 & 0.8 $\pm$ 1.1 & (0.7$\sigma$) \\
C$^{18}$O~(4--3) & 439.0888 & 27 & $-0.2$ $\pm$ 2.0 & ($-0.1\sigma$)  & & CN~(N = 6--5) & 680.2641 & 9 & 0.4 $\pm$ 1.3 & (0.3$\sigma$) \\
C$^{18}$O~(5--4) & 548.8310 & 33 & 2.0 $\pm$ 1.1 & (1.8$\sigma$)  & & SiO~(7--6) & 303.9270 & 19 & 5.3 $\pm$ 4.9 & (1.1$\sigma$) \\
C$^{18}$O~(6--5) & 658.5533 & 14 & 1.0 $\pm$ 1.2 & (0.9$\sigma$)  & & SiO~(8--7) & 347.3306 & 38 & $-1.7$ $\pm$ 2.6 & ($-0.7\sigma$) \\
C$^{18}$O~(7--6) & 768.2515 & 7 & 0.8 $\pm$ 1.1 & (0.7$\sigma$)  & & SiO~(9--8) & 390.7284 & 40 & 0.3 $\pm$ 2.3 & (0.1$\sigma$) \\
C$^{18}$O~(8--7) & 877.9219 & 2 & $-1.0$ $\pm$ 1.6 & ($-0.7\sigma$)  & & SiO~(10--9) & 434.1196 & 25 & 1.2 $\pm$ 2.2 & (0.6$\sigma$) \\
\textsc{[C~i]}~($^3P_1$--$^3P_0$) & 492.1606 & 32 & $\boldsymbol{ 29.0 \pm 2.1}$ & (23.0$\sigma$)  & & SiO~(11--10) & 477.5031 & 35 & $-1.0$ $\pm$ 1.3 & ($-0.8\sigma$) \\
\textsc{[C~i]}~($^3P_2$--$^3P_1$) & 809.3419 & 4 & $\boldsymbol{ 18.8 \pm 1.8}$ & (12.4$\sigma$)  & & SiO~(12--11) & 520.8782 & 40 & 1.2 $\pm$ 1.2 & (1.0$\sigma$) \\
HCN~(3--2) & 265.8864 & 3 & 0.2 $\pm$ 9.2 & (0.0$\sigma$)  & & SiO~(13--12) & 564.2440 & 27 & $-0.8$ $\pm$ 1.1 & ($-0.7\sigma$) \\
HCN~(4--3) & 354.5055 & 40 & $\boldsymbol{ 7.6 \pm 2.6}$ & (3.0$\sigma$)  & & SiO~(14--13) & 607.5994 & 20 & $-0.5$ $\pm$ 1.1 & ($-0.4\sigma$) \\
HCN~(5--4) & 443.1161 & 29 & 3.0 $\pm$ 1.7 & (1.8$\sigma$)  & & SiO~(15--14) & 650.9436 & 14 & $-0.4$ $\pm$ 1.1 & ($-0.4\sigma$) \\
HCN~(6--5) & 531.7164 & 34 & ${ 4.4 \pm 1.2}$ & (3.8$\sigma$)  & & SiO~(16--15) & 694.2754 & 9 & 0.3 $\pm$ 1.3 & (0.2$\sigma$) \\
HCN~(7--6) & 620.3040 & 20 & 1.4 $\pm$ 1.1 & (1.4$\sigma$)  & & SiO~(17--16) & 737.5939 & 6 & 0.1 $\pm$ 1.3 & (0.1$\sigma$) \\
HCN~(8--7) & 708.8770 & 6 & 0.8 $\pm$ 1.4 & (0.5$\sigma$)  & & CS~(6--5) & 293.9122    & 17 & $-10.7$ $\pm$ 5.8 & ($-1.9\sigma$) \\
HCN~(9--8) & 797.4333 & 6 & $-1.0$ $\pm$ 1.2 & ($-0.9\sigma$)  & & CS~(7--6) & 342.8830    & 42 & 3.5 $\pm$ 2.7 & (1.3$\sigma$) \\
HCN~(10--9) & 885.9707 & 2 & $-2.2$ $\pm$ 1.5 & ($-1.5\sigma$)  & & CS~(8--7) & 391.8470    & 39 & $-0.2$ $\pm$ 2.3 & ($-0.1\sigma$) \\
HNC~(3--2) & 271.9811 & 4 & 8.7 $\pm$ 11.2 & (0.8$\sigma$)  & & CS~(10--9) & 489.7510 & 33 & 1.0 $\pm$ 1.3 & (0.8$\sigma$) \\
HNC~(4--3) & 362.6303 & 35 & 0.3 $\pm$ 3.0 & (0.1$\sigma$)  & & CS~(11--10) & 538.6888 & 33 & $-0.2$ $\pm$ 1.2 & ($-0.1\sigma$) \\
HNC~(5--4) & 453.2699 & 36 & 3.4 $\pm$ 1.4 & (2.4$\sigma$)  & & CS~(12--11) & 587.6162 & 23 & 1.0 $\pm$ 1.1 & (0.9$\sigma$) \\
HNC~(6--5) & 543.8976 & 34 & 1.8 $\pm$ 1.2 & (1.6$\sigma$)  & & CS~(13--12) & 636.5318 & 15 & $-0.6$ $\pm$ 1.2 & ($-0.5\sigma$) \\
HNC~(7--6) & 634.5108 & 17 & 0.4 $\pm$ 1.1 & (0.3$\sigma$)  & & CS~(14--13) & 685.4348 & 10 & 1.0 $\pm$ 1.2 & (0.8$\sigma$) \\
HNC~(8--7) & 725.1073 & 6 & $-0.3$ $\pm$ 1.3 & ($-0.2\sigma$)  & & CS~(15--14) & 734.3240 & 6 & 0.8 $\pm$ 1.3 & (0.6$\sigma$) \\
HNC~(9--8) & 815.6847 & 3 & $-1.1$ $\pm$ 1.6 & ($-0.7\sigma$)  & & NH$_3$~(1$_0$--0$_0$) & 572.4982 & 25 & 1.0 $\pm$ 1.0 & (1.0$\sigma$) \\
HCO$^+$~(3--2) & 267.5576 & 4 & 5.1 $\pm$ 8.3 & (0.6$\sigma$)  & & N$_2$H$^+$~(3--2) & 279.5117 & 8 & 1.4 $\pm$ 9.0 & (0.2$\sigma$) \\
HCO$^+$~(4--3) & 356.7342 & 40 & 3.4 $\pm$ 2.5 & (1.4$\sigma$)  & & N$_2$H$^+$~(4--3) & 372.6725    & 39 & $-1.6$ $\pm$ 2.3 & ($-0.7\sigma$) \\
HCO$^+$~(5--4) & 445.9029 & 31 & 4.5 $\pm$ 1.5 & (3.0$\sigma$)  & & N$_2$H$^+$~(5--4) & 465.8250 & 32 & 0.1 $\pm$ 1.5 & (0.1$\sigma$) \\
HCO$^+$~(6--5) & 535.0616 & 33 & 1.6 $\pm$ 1.2 & (1.3$\sigma$)  & & N$_2$H$^+$~(6--5) & 558.9667    & 27 & $-2.1$ $\pm$ 1.3 & ($-1.7\sigma$) \\
HCO$^+$~(7--6) & 624.2085 & 17 & 0.6 $\pm$ 1.1 & (0.5$\sigma$)  & & N$_2$H$^+$~(7--6) & 652.0959    & 15 & $-0.8$ $\pm$ 1.1 & ($-0.7\sigma$) \\
HCO$^+$~(8--7) & 713.3414 & 5 & 0.1 $\pm$ 1.4 & (0.0$\sigma$)  & & N$_2$H$^+$~(8--7) & 745.2103    & 6 & 1.9 $\pm$ 1.3 & (1.5$\sigma$) \\
HCO$^+$~(9--8) & 802.4582 & 5 & $-2.5$ $\pm$ 1.4 & ($-1.9\sigma$)  & & CCH~(3--2) & 262.0042    & 2 & 1.0 $\pm$ 9.4 & (0.1$\sigma$) \\
HCO$^+$~(10--9) & 891.5573 & 2 & $-0.6$ $\pm$ 1.5 & ($-0.4\sigma$)  & & CCH~(4--3) & 349.3387    & 40 & 1.1 $\pm$ 2.6 & (0.4$\sigma$) \\
HOC$^+$~(3--2) & 268.4510 & 4 & $-1.4$ $\pm$ 8.5 & ($-0.2\sigma$)  & & CCH~(5--4) & 436.6604    & 27 & $-4.0$ $\pm$ 2.1 & ($-1.9\sigma$) \\
HOC$^+$~(4--3) & 357.9219 & 40 & $-5.0$ $\pm$ 2.4 & ($-2.1\sigma$)  & & CCH~(6--5) & 523.9704    & 37 & $-0.9$ $\pm$ 1.2 & ($-0.7\sigma$) \\
HOC$^+$~(5--4) & 447.3818 & 30 & $-0.7$ $\pm$ 1.5 & ($-0.5\sigma$)  & & CCH~(7--6) & 611.2650 & 20 & $-0.1$ $\pm$ 1.1 & ($-0.1\sigma$) \\
HOC$^+$~(6--5) & 536.8279 & 31 & ${ 7.6 \pm 1.3}$ & (6.4$\sigma$)  & & CCH~(8--7) & 698.5416    & 7 & 0.3 $\pm$ 1.4 & (0.2$\sigma$) \\
HOC$^+$~(7--6) & 626.2575 & 17 & $-0.0$ $\pm$ 1.1 & ($-0.0\sigma$)  & & H21$\alpha$ & 662.4042    & 13 & 0.7 $\pm$ 1.2 & (0.6$\sigma$) \\
HOC$^+$~(8--7) & 715.6679 & 6 & 0.3 $\pm$ 1.4 & (0.2$\sigma$)  & & H22$\alpha$ & 577.8964    & 27 & 0.3 $\pm$ 1.0 & (0.3$\sigma$) \\
HOC$^+$~(9--8) & 805.0563 & 4 & 0.7 $\pm$ 1.5 & (0.5$\sigma$)  & & H23$\alpha$ & 507.1755    & 35 & $-0.8$ $\pm$ 1.1 & ($-0.8\sigma$) \\
H$_2$O~(5$_{1, 5}$--4$_{2, 2}$) & 325.1529 & 38 & $-5.8$ $\pm$ 3.4 & ($-1.7\sigma$)  & & H24$\alpha$ & 447.5403    & 30 & 0.1 $\pm$ 1.5 & (0.0$\sigma$) \\
H$_2$O~(4$_{1, 4}$--3$_{2, 1}$) & 380.1974 & 42 & 0.7 $\pm$ 2.2 & (0.3$\sigma$)  & & H25$\alpha$ & 396.9008 & 35 & $-1.6$ $\pm$ 2.4 & ($-0.7\sigma$) \\
H$_2$O~(4$_{2, 3}$--3$_{3, 0}$) & 448.0011 & 31 & 1.8 $\pm$ 1.5 & (1.2$\sigma$)  & & H26$\alpha$ & 353.6227 & 41 & 5.2 $\pm$ 2.5 & (2.1$\sigma$) \\
H$_2$O~(5$_{3, 3}$--4$_{4, 0}$) & 474.6891 & 33 & $-2.2$ $\pm$ 1.3 & ($-1.6\sigma$)  & & H27$\alpha$ & 316.4154 & 29 & $-4.7$ $\pm$ 4.0 & ($-1.2\sigma$) \\
H$_2$O~(1$_{1, 0}$--1$_{0, 1}$) & 556.9360 & 30 & $-1.0$ $\pm$ 1.2 & ($-0.8\sigma$)  & & H28$\alpha$ & 284.2506 & 10 & 9.0 $\pm$ 8.0 & (1.1$\sigma$) \\
H$_2$O~(2$_{1, 1}$--2$_{0, 2}$) & 752.0331 & 5 & $\boldsymbol{10.6 \pm 1.4}$ & (8.5$\sigma$)  & & CH$^+$ & 835.0789 & 2 & $-0.5$ $\pm$ 1.7 & ($-0.3\sigma$) \\
H$_2$O$^+$~604 & 604.6786 & 22 & 0.6 $\pm$ 1.1 & (0.6$\sigma$) \\
\hline
\end{tabular}
\raggedright \justify \vspace{-0.2cm}
\textbf{Notes:} Lines in bold-face indicate $> 3\sigma$ detections. Note that the apparent HCN~(6--5) and HOC$^+$~(6--5) ``detections'' are due to line confusion with CH~532 and 536.
\end{table}




% Old version
% CO (2--1) & 230.5380 & 2 & $\boldsymbol{ 128.8 \pm 14.9}$ & (9.9$\sigma$) & H$_2$O$^+$ 604 & 604.6786 & 22 & 0.1 $\pm$ 1.1 & (0.1$\sigma$) \\
% CO (3--2) & 345.7960 & 42 & $\boldsymbol{ 98.2 \pm 6.1}$ & (37.9$\sigma$) & H$_2$O$^+$ 607 & 607.2273 & 20 & $-0.5$ $\pm$ 1.1 & ($-0.4$$\sigma$) \\
% CO (4--3) & 461.0408 & 35 & $\boldsymbol{ 74.0 \pm 4.4}$ & (53.7$\sigma$) & H$_2$O$^+$ 631 & 631.7241 & 17 & 0.0 $\pm$ 1.1 & (0.0$\sigma$) \\
% CO (5--4) & 576.2679 & 27 & $\boldsymbol{ 69.5 \pm 4.0}$ & (67.5$\sigma$) & H$_2$O$^+$ 634 & 634.2729 & 17 & $-0.1$ $\pm$ 1.1 & ($-0.1$$\sigma$) \\
% CO (6--5) & 691.4731 & 10 & $\boldsymbol{ 50.4 \pm 3.1}$ & (39.4$\sigma$) & H$_2$O$^+$ 721 & 721.9274 & 6 & $-3.4$ $\pm$ 1.5 & ($-2.2$$\sigma$) \\
% CO (7--6) & 806.8984 & 4 & $\boldsymbol{ 38.2 \pm 2.6}$ & (25.1$\sigma$) & H$_2$O$^+$ 742 & 742.1090 & 5 & 1.8 $\pm$ 1.5 & (1.2$\sigma$) \\
% $^{13}$CO (2--1) & 220.3987 & 1 & 6.6 $\pm$ 18.4 & (0.4$\sigma$) & H$_2$O$^+$ 746 & 746.5417 & 5 & $\boldsymbol{ 5.6 \pm 1.4}$ & (4.2$\sigma$) \\
% $^{13}$CO (3--2) & 330.5880 & 41 & 4.1 $\pm$ 3.2 & (1.3$\sigma$) & H$_2$O$^+$ 761 & 761.8188 & 6 & 1.5 $\pm$ 1.2 & (1.3$\sigma$) \\
% $^{13}$CO (4--3) & 440.7652 & 28 & 2.4 $\pm$ 2.0 & (1.2$\sigma$) & LiH (1--0) & 443.9529 & 30 & $-2.7$ $\pm$ 1.7 & ($-1.6$$\sigma$) \\
% $^{13}$CO (5--4) & 550.9263 & 29 & 2.0 $\pm$ 1.2 & (1.7$\sigma$) & CH 536 & 536.7614 & 31 & $\boldsymbol{ 8.2 \pm 1.3}$ & (6.8$\sigma$) \\
% $^{13}$CO (6--5) & 661.0673 & 14 & 2.7 $\pm$ 1.2 & (2.3$\sigma$) & OH 425 & 425.0363 & 25 & 0.7 $\pm$ 2.5 & (0.3$\sigma$) \\
% $^{13}$CO (7--6) & 771.1841 & 7 & $-0.2$ $\pm$ 1.0 & ($-0.2$$\sigma$) & OH 446 & 446.2910 & 31 & 2.0 $\pm$ 1.5 & (1.3$\sigma$) \\
% $^{13}$CO (8--7) & 881.2728 & 2 & 1.8 $\pm$ 1.5 & (1.2$\sigma$) & CN (N = 3--2) & 340.2478 & 41 & 1.9 $\pm$ 2.8 & (0.7$\sigma$) \\
% C$^{18}$O (2--1) & 219.5603 & 1 & $-25.1$ $\pm$ 19.8 & ($-1.3$$\sigma$) & CN (N = 4--3) & 453.6067 & 36 & 2.0 $\pm$ 1.4 & (1.4$\sigma$) \\
% C$^{18}$O (3--2) & 329.3305 & 42 & 2.4 $\pm$ 3.2 & (0.8$\sigma$) & CN (N = 5--4) & 566.9470 & 26 & 1.2 $\pm$ 1.1 & (1.1$\sigma$) \\
% C$^{18}$O (4--3) & 439.0888 & 27 & 0.0 $\pm$ 2.0 & (0.0$\sigma$) & CN (N = 6--5) & 680.2641 & 9 & 1.1 $\pm$ 1.3 & (0.9$\sigma$) \\
% C$^{18}$O (5--4) & 548.8310 & 33 & 2.3 $\pm$ 1.1 & (2.0$\sigma$) & SiO (7--6) & 303.9270 & 19 & 4.6 $\pm$ 4.9 & (0.9$\sigma$) \\
% C$^{18}$O (6--5) & 658.5533 & 14 & 2.5 $\pm$ 1.2 & (2.1$\sigma$) & SiO (8--7) & 347.3306 & 38 & $-1.6$ $\pm$ 2.6 & ($-0.6$$\sigma$) \\
% C$^{18}$O (7--6) & 768.2515 & 7 & 1.5 $\pm$ 1.1 & (1.4$\sigma$) & SiO (9--8) & 390.7284 & 40 & 0.4 $\pm$ 2.3 & (0.2$\sigma$) \\
% C$^{18}$O (8--7) & 877.9219 & 2 & 1.8 $\pm$ 1.6 & (1.1$\sigma$) & SiO (10--9) & 434.1196 & 25 & 1.3 $\pm$ 2.2 & (0.6$\sigma$) \\
% \textsc{[C~i]} ($^3P_1$--$^3P_0$) & 492.1606 & 32 & $\boldsymbol{ 29.1 \pm 2.1}$ & (23.1$\sigma$) & SiO (11--10) & 477.5031 & 35 & $-1.2$ $\pm$ 1.3 & ($-0.9$$\sigma$) \\
% \textsc{[C~i]} ($^3P_2$--$^3P_1$) & 809.3419 & 4 & $\boldsymbol{ 19.0 \pm 1.9}$ & (12.3$\sigma$) & SiO (12--11) & 520.8782 & 40 & 1.0 $\pm$ 1.2 & (0.9$\sigma$) \\
% HCN (3--2) & 265.8864 & 3 & 0.7 $\pm$ 9.2 & (0.1$\sigma$) & SiO (13--12) & 564.2440 & 27 & $-0.4$ $\pm$ 1.1 & ($-0.3$$\sigma$) \\
% HCN (4--3) & 354.5055 & 40 & $\boldsymbol{ 8.0 \pm 2.6}$ & (3.1$\sigma$) & SiO (14--13) & 607.5994 & 20 & $-0.8$ $\pm$ 1.1 & ($-0.7$$\sigma$) \\
% HCN (5--4) & 443.1161 & 29 & 2.8 $\pm$ 1.7 & (1.6$\sigma$) & SiO (15--14) & 650.9436 & 14 & 1.0 $\pm$ 1.2 & (0.9$\sigma$) \\
% HCN (6--5) & 531.7164 & 34 & $\boldsymbol{ 4.5 \pm 1.2}$ & (3.8$\sigma$) & SiO (16--15) & 694.2754 & 9 & $-0.2$ $\pm$ 1.3 & ($-0.2$$\sigma$) \\
% HCN (7--6) & 620.3040 & 20 & 1.7 $\pm$ 1.1 & (1.6$\sigma$) & SiO (17--16) & 737.5939 & 6 & 0.1 $\pm$ 1.3 & (0.1$\sigma$) \\
% HCN (8--7) & 708.8770 & 6 & $-0.6$ $\pm$ 1.4 & ($-0.4$$\sigma$) & CS (6--5) & 293.9122    & 17 & $-11.7$ $\pm$ 5.8 & ($-2.0$$\sigma$) \\
% HCN (9--8) & 797.4333 & 6 & 0.2 $\pm$ 1.2 & (0.1$\sigma$) & CS (7--6) & 342.8830    & 42 & 3.5 $\pm$ 2.7 & (1.3$\sigma$) \\
% HCN (10--9) & 885.9707 & 2 & 1.0 $\pm$ 1.5 & (0.7$\sigma$) & CS (8--7) & 391.8470    & 39 & -0.0 $\pm$ 2.3 & (0.0$\sigma$) \\
% HNC (3--2) & 271.9811 & 4 & 9.0 $\pm$ 11.2 & (0.8$\sigma$) & CS (10--9) & 489.7510 & 33 & 1.0 $\pm$ 1.3 & (0.8$\sigma$) \\
% HNC (4--3) & 362.6303 & 35 & 0.4 $\pm$ 3.0 & (0.1$\sigma$) & CS (11--10) & 538.6888 & 33 & 0.3 $\pm$ 1.2 & (0.2$\sigma$) \\
% HNC (5--4) & 453.2699 & 36 & 3.1 $\pm$ 1.4 & (2.2$\sigma$) & CS (12--11) & 587.6162 & 23 & 1.2 $\pm$ 1.1 & (1.1$\sigma$) \\
% HNC (6--5) & 543.8976 & 34 & 2.2 $\pm$ 1.2 & (1.9$\sigma$) & CS (13--12) & 636.5318 & 15 & 0.0 $\pm$ 1.2 & (0.0$\sigma$) \\
% HNC (7--6) & 634.5108 & 17 & 1.0 $\pm$ 1.1 & (0.9$\sigma$) & CS (14--13) & 685.4348 & 10 & 1.3 $\pm$ 1.2 & (1.1$\sigma$) \\
% HNC (8--7) & 725.1073 & 6 & $0.9$ $\pm$ 1.4 & ($-0.7$$\sigma$) & CS (15--14) & 734.3240 & 6 & 0.7 $\pm$ 1.3 & (0.5$\sigma$) \\
% HNC (9--8) & 815.6847 & 3 & $-0.9$ $\pm$ 1.6 & ($-0.6$$\sigma$) & NH$_3$ (1$_0$--0$_0$) & 572.4982 & 25 & 1.1 $\pm$ 1.0 & (1.1$\sigma$) \\
% HCO$^+$ (3--2) & 267.5576 & 4 & 5.5 $\pm$ 8.3 & (0.7$\sigma$) & N$_2$H$^+$ (3--2) & 279.5117 & 8 & 1.5 $\pm$ 9.0 & (0.2$\sigma$) \\
% HCO$^+$ (4--3) & 356.7342 & 40 & 3.8 $\pm$ 2.5 & (1.5$\sigma$) & N$_2$H$^+$ (4--3) & 372.6725    & 39 & $-1.6$ $\pm$ 2.3 & ($-0.7$$\sigma$) \\
% HCO$^+$ (5--4) & 445.9029 & 31 & 4.1 $\pm$ 1.5 & (2.7$\sigma$) & N$_2$H$^+$ (5--4) & 465.8250 & 32 & $-0.3$ $\pm$ 1.5 & ($-0.2$$\sigma$) \\
% HCO$^+$ (6--5) & 535.0616 & 33 & 1.8 $\pm$ 1.2 & (1.5$\sigma$) & N$_2$H$^+$ (6--5) & 558.9667    & 27 & $-1.5$ $\pm$ 1.3 & ($-1.2$$\sigma$) \\
% HCO$^+$ (7--6) & 624.2085 & 17 & 0.8 $\pm$ 1.1 & (0.7$\sigma$) & N$_2$H$^+$ (7--6) & 652.0959    & 15 & 0.7 $\pm$ 1.1 & (0.6$\sigma$) \\
% HCO$^+$ (8--7) & 713.3414 & 5 & $-1.2$ $\pm$ 1.4 & ($-0.9$$\sigma$) & N$_2$H$^+$ (8--7) & 745.2103    & 6 & 2.5 $\pm$ 1.4 & (1.9$\sigma$) \\
% HCO$^+$ (8--7) & 802.4582 & 5 & $-2.0$ $\pm$ 1.4 & ($-1.5$$\sigma$) & CCH (3--2) & 262.0042    & 2 & 1.5 $\pm$ 9.4 & (0.2$\sigma$) \\
% HCO$^+$ (8--7) & 891.5573 & 2 & 3.0 $\pm$ 1.5 & (2.0$\sigma$) & CCH (4--3) & 349.3387    & 40 & 1.3 $\pm$ 2.6 & (0.5$\sigma$) \\
% HOC$^+$ (3--2) & 268.4510 & 4 & $-1.0$ $\pm$ 8.5 & ($-0.1$$\sigma$) & CCH (5--4) & 436.6604    & 27 & $-3.8$ $\pm$ 2.1 & ($-1.8$$\sigma$) \\
% HOC$^+$ (4--3) & 357.9219 & 40 & $-4.8$ $\pm$ 2.4 & ($-2.0$$\sigma$) & CCH (6--5) & 523.9704    & 37 & $-1.1$ $\pm$ 1.2 & ($-0.9$$\sigma$) \\
% HOC$^+$ (5--4) & 447.3818 & 30 & $-1.1$ $\pm$ 1.5 & ($-0.7$$\sigma$) & CCH (7--6) & 611.2650 & 20 & $-0.3$ $\pm$ 1.1 & ($-0.3$$\sigma$) \\
% HOC$^+$ (6--5) & 536.8279 & 31 & $\boldsymbol{ 7.9 \pm 1.3}$ & (6.6$\sigma$) & CCH (8--7) & 698.5416    & 7 & $-0.5$ $\pm$ 1.4 & ($-0.4$$\sigma$) \\
% HOC$^+$ (7--6) & 626.2575 & 17 & 0.3 $\pm$ 1.1 & (0.3$\sigma$) & H21$\alpha$ & 662.4042    & 13 & 2.3 $\pm$ 1.2 & (1.9$\sigma$) \\
% HOC$^+$ (8--7) & 715.6679 & 6 & $-0.8$ $\pm$ 1.4 & ($-0.6$$\sigma$) & H22$\alpha$ & 577.8964    & 27 & 0.6 $\pm$ 1.0 & (0.5$\sigma$) \\
% HOC$^+$ (9--8) & 805.0563 & 4 & 0.7 $\pm$ 1.5 & (0.5$\sigma$) & H23$\alpha$ & 507.1755    & 35 & $-0.7$ $\pm$ 1.1 & ($-0.7$$\sigma$) \\
% H$_2$O (5$_{1, 5}$--4$_{2, 2}$) & 325.1529 & 38 & $-6.1$ $\pm$ 3.4 & ($-1.8$$\sigma$) & H24$\alpha$ & 447.5403    & 30 & $-0.4$ $\pm$ 1.5 & ($-0.2$$\sigma$) \\
% H$_2$O (4$_{1, 4}$--3$_{2, 1}$) & 380.1974 & 42 & 0.8 $\pm$ 2.2 & (0.4$\sigma$) & H25$\alpha$ & 396.9008 & 35 & $-1.4$ $\pm$ 2.4 & ($-0.6$$\sigma$) \\
% H$_2$O (4$_{2, 3}$--3$_{3, 0}$) & 448.0011 & 31 & 1.4 $\pm$ 1.5 & (0.9$\sigma$) & H26$\alpha$ & 353.6227 & 41 & 5.4 $\pm$ 2.5 & (2.2$\sigma$) \\
% H$_2$O (5$_{3, 3}$--4$_{4, 0}$) & 474.6891 & 33 & $-2.3$ $\pm$ 1.3 & ($-1.7$$\sigma$) & H27$\alpha$ & 316.4154 & 29 & $-5.1$ $\pm$ 4.0 & ($-1.3$$\sigma$) \\
% H$_2$O (1$_{1, 0}$--1$_{0, 1}$) & 556.9360 & 30 & $-0.5$ $\pm$ 1.2 & ($-0.4$$\sigma$) & H28$\alpha$ & 284.2506 & 10 & 9.0 $\pm$ 8.0 & (1.1$\sigma$) \\
% H$_2$O (2$_{1, 1}$--2$_{0, 2}$) & 752.0331 & 5 & $\boldsymbol{ 11.3 \pm 1.4}$ & (8.9$\sigma$) & CH$^+$ & 835.0789 & 2 & $-0.3$ $\pm$ 1.8 & ($-0.2$$\sigma$) \\
